On the Use of Two-Way Fixed Effects Models for Policy Evaluation During Pandemics

In the context of the Covid-19 pandemic, multiple studies rely on two-way fixed effects (FE) models to assess the impact of mitigation policies on health outcomes. Building on the SIRD model of disease transmission, I show that FE models tend to be misspecified for three reasons. First, despite misleading common trends in the pre-treatment period, the parallel trends assumption generally does not hold. Second, heterogeneity in infection rates and infected populations across regions cannot be accounted for by region-specific fixed effects, nor by conditioning on observable time-varying confounders. Third, epidemiological theory predicts heterogeneous treatment effects across regions and over time. Via simulations, I find that the bias resulting from model misspecification can be substantial, in magnitude and sometimes in sign. Overall, my results caution against the use of FE models for mitigation policy evaluation.

==> On the Use of Two-Way Fixed Effects Models for Policy Evaluation During Pandemics/tables/summary_results.tex <==
% Please add the following required packages to your document preamble:
\renewcommand{\arraystretch}{1.3}
\begin{table}[h!] 
\begin{center}
\begin{tabular}{c|l|l|ccc}
\hline
Policy                       & Model       & Dependent Variable & Estimate & S.E. & RMSE       \\ \hline
\multirow{6}{*}{Inefficient (0\%)} &  DID & Cumulative & 0.0117 & 0.0027 & 29949.3922 \\ 
 & DID & Log & 0.0848 & 0.0226 & 102105.3559 \\ 
 & DID & Delta Log & -0.0025 & 0.0006 & 213778.9838 \\
\cline{2-6}
 & Event Study & Cumulative & 0.0004 & 0.0075 & 34069.9416 \\ 
 & Event Study & Log & 0.0019 & 0.0748 & 101639.7259 \\ 
 & Event Study & Delta Log & 0.0003 & 0.0019 & 224595.3068 \\ 
                             \hline
\multirow{6}{*}{Efficient (-10\%)} & DID & Cumulative & -0.0077 & 0.0026 & 39123.6259 \\ 
& DID & Log & -0.1633 & 0.0219 & 102863.3005 \\ 
 & DID & Delta Log & -0.0090 & 0.0006 & 198567.7457 \\ 
\cline{2-6}
 & Event Study & Cumulative & -0.0000 & 0.0072 & 34650.7758 \\ 
 & Event Study & Log & -0.0982 & 0.0703 & 94776.0034 \\ 
 & Event Study & Delta Log & -0.0999 & 0.0018 & 209971.6188 \\ \hline
\end{tabular}
\vspace{0.2cm}
\caption{Summary of Simulation Results}
\label{tab:simresults}
\end{center}
\footnotesize
\renewcommand{\baselineskip}{11pt}
\textbf{Note:} I estimate two models on all three dependent variables used in the literature: a FE linear regression model with constant treatment effects, and a dynamic FE linear regression model (an `event study'). I also consider two scenarios. In the first scenario, the mitigation policy is inefficient and does not affect the infection rate. In the second scenario, it decreases the infection rate by 10\%. For each specification, I present the point estimate, its associated standard error, and the root mean squared error. For clarity, the latter is always computed based on the number of cumulative new infectious individuals. In the case of event study estimates, the point estimate is the estimated effect of the mitigation policy `on impact'. For completeness, the event-study graphs are provided in Appendix A.
\end{table}
